Percolation properties of the neutron population in nuclear reactors

Reactor physics aims at studying the neutron population in a reactor core under the influence of feedback mechanisms, such as the Doppler temperature effect. Numerical schemes to calculate macroscopic properties emerging from such coupled stochastic systems however require to define intermediate quantities (e.g. the temperature field), which are bridging the gap between the stochastic neutron field and the deterministic feedback. By interpreting the branching random walk of neutrons in fissile media under the influence of a feedback mechanism as a directed percolation process and by leveraging on the statistical field theory of birth death processes, we will build a stochastic model of neutron transport theory and of reactor physics. The critical exponents of this model, combined to the analysis of the resulting field equation involving a fractional Laplacian will show that the critical diffusion equation cannot adequately describe the spatial distribution of the neutron population and shifts instead to a critical super-diffusion equation. The analysis of this equation will reveal that non-negligible departure from mean field behavior might develop in reactor cores, questioning the attainable accuracy of the numerical schemes currently used by the nuclear industry.

==> old/4_two_species_old.tex <==
\section{Two species model - The importance of being delayed}

Another key element in the modelling  of the temporal behaviour of the neutron population in a nuclear reactor is the role played by the precursor population of delayed neutrons $M(t)$. Precursors are unstable fission products resulting from the fission of heavy nuclides. Their further decay, with rate $\lambda_D$, into a stable isotope result in the emission of a fraction $\beta$ of the total neutron population. 

Including the coupling between the neutron and precursor populations, the point-like model studied up to now becomes (with $r = \rho - \beta)$, 

\begin{equation}
\begin{cases}
        \cfrac{d N(t)}{dt} & = r N(t) + \lambda_D M(t) + \eta(t), \\
         \\
    \cfrac{d M(t)}{dt} & = \beta N(t) - \lambda_D M(t) + \zeta(t) ,
\end{cases}
\end{equation}
where external sources have been neglected, for simplicity. For the same reason, and although this does not correspond to what would have been expected on physical ground, the stochastic terms $\eta$ and $\zeta$ will be considered independent in the following. 

The derivation of the response functional associated to this coupled system of equations follows exactly the recipe described in section \ref{sec:FieldFormulation}. Four independent fields $\Nt \Mt M$ and $N$ are now introduced into the theory and the response functional can be written $\mathcal{S} = \mathcal{S}_{\text{neut.}} + \mathcal{S}_{\text{prec}}$, with,
\begin{eqnarray}
     \mathcal{S}_{\text{neut.}} & = & \int \left\{\Nt(t)  \left( \frac{d}{dt} - r \right)N(t) \right. \nonumber\\ 
     & & \left. -  \lambda_D \Nt(t) M(t) - \lambda_1 \Nt^2(t) N(t) \right\} dt
\end{eqnarray}
and
\begin{eqnarray}
     \mathcal{S}_{\text{prec.}} & = & \int \left\{ \,\Mt(t)  \left( \frac{d}{dt} + \lambda_D \right)M(t) \right. \nonumber\\
     & & \left. - \beta \Mt(t) N(t) - \lambda_2 \Mt^2(t) M(t) \right\} dt.
\end{eqnarray}
The coupling between these two functional renders the perturbative calculations of observables much more involved. One has for instance to take into account the decay of precursors into neutrons or the creation of precursors following a fission event. This translate into a more general form for the basic objects of the theory: the propagators that must be taken into account now reads,  
\begin{widetext}
\begin{eqnarray}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \Sigma_{NN}(t,t')  & =&  \begin{tikzpicture}[baseline=(a)]
    \begin{feynman}[small, inline=(a)]
      \vertex (a);
      \vertex [right=0.5 cm of a,blob](b) {};
      \vertex [right=0.7 cm of b](o1);
    \diagram* {
    (a) --  (b) -- (o1)
    };
    \end{feynman}
  \end{tikzpicture} =
     \begin{tikzpicture}[baseline=(a)]
    \begin{feynman}[inline=(a)]
      \vertex (a);
      \vertex [right=of a](o1);
    \diagram* {
    (a) -- (o1)
    };
    \end{feynman}
  \end{tikzpicture}
  + \beta \, \lambda_D \,
    \begin{tikzpicture}[baseline=(a)]
    \begin{feynman}[small, inline=(a)]
      \vertex (a);
      \vertex [right=0.5 cm of a,dot](b) {};
      \vertex [right=0.7 cm of b,dot](c) {};
      \vertex [right=0.5 cm of c](o1);
    \diagram* {
    (a) -- (b) ,
    (b)--[scalar] (c),
    (c) -- (o1)
    };
    \end{feynman}
  \end{tikzpicture}
  + \left( \beta \, \lambda_D  \right)^2
  \begin{tikzpicture}[baseline=(a)]
    \begin{feynman}[small, inline=(a)]
      \vertex (a);
      \vertex [right=0.5 cm of a,dot](b) {};
      \vertex [right=0.7 cm of b,dot](c) {};
      \vertex [right=0.7 cm of c,dot](d) {};
      \vertex [right=0.7 cm of d,dot](e) {};
      \vertex [right=0.5 cm of e](o1);
    \diagram* {
    (a) -- (b) ,
    (b)--[scalar] (c),
    (c) -- (d) ,
    (d)--[scalar] (e),
    (e) -- (o1)
    };
    \end{feynman}
  \end{tikzpicture}
  + ... \, , \, \nonumber\\ & & \nonumber\\
  & = & e^{r(t-t')} + e^{r(t-t')} \beta \lambda_D \int_{t'}^t dt_1 e^{-(r + \lambda_D) t_1} \int_{t'}^{t_1} dt_2 e^{(r+\lambda_D) t_2} + ...\, , \, \nonumber\\ & & \nonumber\\
  & = &  e^{r(t-t')} \left\{1 + \int_{0}^{t-t'}\sqrt{\frac{\beta\lambda_D(t-t'-\tau)}{\tau}}e^{-(r + \lambda_D)\tau} I_1\left(2\sqrt{\beta\lambda_D \tau (t-t'-\tau)}\right) d\tau \right\} \\\nonumber \\ \nonumber \\
  & = & e^{ r (t-t')} e^{-(r+\lambda_D)(t - t')/2} \left\{ \cosh\left( \frac{ (r+\lambda_D)(t-t')}{2} \sqrt{ 1 + \frac{4 \beta \lambda_D}{(r+\lambda_D)^2}   }\right) \right\}\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \Sigma_{MM}(t,t')  & =&  \begin{tikzpicture}[baseline=(a)]
    \begin{feynman}[small, inline=(a)]
      \vertex (a);
      \vertex [right=0.5 cm of a,blob](b) {};
      \vertex [right=0.7 cm of b](o1);
    \diagram* {
    (a) -- [scalar] (b) --[scalar] (o1)
    };
    \end{feynman}
  \end{tikzpicture} =
     \begin{tikzpicture}[baseline=(a)]
    \begin{feynman}[inline=(a)]
      \vertex (a);
      \vertex [right=of a](o1);
    \diagram* {
    (a) --[scalar] (o1)
    };
    \end{feynman}
  \end{tikzpicture}
  + \beta \, \lambda_D \,
    \begin{tikzpicture}[baseline=(a)]
    \begin{feynman}[small, inline=(a)]
      \vertex (a);
      \vertex [right=0.5 cm of a,dot](b) {};
      \vertex [right=0.7 cm of b,dot](c) {};
      \vertex [right=0.5 cm of c](o1);
    \diagram* {
    (a) --[scalar] (b) ,
    (b)-- (c),
    (c) --[scalar] (o1)
    };
    \end{feynman}
  \end{tikzpicture}
  + \left( \beta \, \lambda_D  \right)^2
  \begin{tikzpicture}[baseline=(a)]
    \begin{feynman}[small, inline=(a)]
      \vertex (a);
      \vertex [right=0.5 cm of a,dot](b) {};
      \vertex [right=0.7 cm of b,dot](c) {};
      \vertex [right=0.7 cm of c,dot](d) {};
      \vertex [right=0.7 cm of d,dot](e) {};
      \vertex [right=0.5 cm of e](o1);
    \diagram* {
    (a) --[scalar] (b) ,
    (b)-- (c),
    (c) --[scalar] (d) ,
    (d)-- (e),
    (e) --[scalar] (o1)
    };
    \end{feynman}
  \end{tikzpicture}
  + ... \, , \, \nonumber\\ & & \nonumber\\
  & = & e^{-\lambda_d(t-t')} \left\{1 + \int_{0}^{t-t'}\sqrt{\frac{\beta\lambda_d(t-t'-\tau)}{\tau}}e^{(r + \lambda_d)\tau} I_1\left(2\sqrt{\beta\lambda_d \tau (t-t'-\tau)}\right) d\tau \right\} \\ \nonumber \\ \nonumber \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \Sigma_{NM}(t,t')  & =&  \begin{tikzpicture}[baseline=(a)]
    \begin{feynman}[small, inline=(a)]
      \vertex (a);
      \vertex [right=0.5 cm of a,blob](b) {};
      \vertex [right=0.7 cm of b](o1);
    \diagram* {
    (a) -- [scalar] (b) --(o1)
    };
    \end{feynman}
  \end{tikzpicture} = \beta \left\{ \begin{tikzpicture}[baseline=(a)]
    \begin{feynman}[inline=(a)]
      \vertex (a);
      \vertex [right=of a,dot](b) {};
      \vertex [right=of b](o1);
    \diagram* {
    (a) --[scalar] (b),
    (b) -- (o1)
    };
    \end{feynman}
  \end{tikzpicture}
  + \beta \, \lambda_D \, \, 
    \begin{tikzpicture}[baseline=(a)]
    \begin{feynman}[inline=(a)]
      \vertex (a);
      \vertex [right=of a,dot](b) {};
      \vertex [right=of b,dot](c) {};
      \vertex [right=of c,dot](d) {};
      \vertex [right=of d](o1);
    \diagram* {
    (a) --[scalar] (b) ,
    (b)-- (c),
    (c)-- [scalar] (d),
    (d) -- (o1)
    };
    \end{feynman}
  \end{tikzpicture}
  + ...\right\} \nonumber\\ & & \nonumber\\
  & = & \beta e^{-\lambda_d(t-t')} \int_{0}^{t-t'} e^{(r + \lambda_d)\tau} I_0\left(2\sqrt{\beta\lambda_d \tau (t-t'-\tau)}\right) d\tau
  \end{eqnarray}
\end{widetext}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 \begin{widetext}
 \begin{eqnarray}
   \Sigma_{MN}(t,t') & = & \begin{tikzpicture}[baseline=(a)]
    \begin{feynman}[small, inline=(a)]
      \vertex (a);
      \vertex [right=0.5 cm of a,blob](b) {};
      \vertex [right=0.8 cm of b](o1);
    \diagram* {
    (a) --  (b) -- [scalar] (o1)
    };
    \end{feynman}
  \end{tikzpicture} = \lambda_D \left\{ \begin{tikzpicture}[baseline=(a)]
    \begin{feynman}[inline=(a)]
      \vertex (a);
      \vertex [right=of a,dot](b) {};
      \vertex [right=of b](o1);
    \diagram* {
    (a) -- (b),
    (b) --[scalar] (o1)
    };
    \end{feynman}
  \end{tikzpicture}
  + \beta \, \lambda_D \, \, 
    \begin{tikzpicture}[baseline=(a)]
    \begin{feynman}[inline=(a)]
      \vertex (a);
      \vertex [right=of a,dot](b) {};
      \vertex [right=of b,dot](c) {};
      \vertex [right=of c,dot](d) {};
      \vertex [right=of d](o1);
    \diagram* {
    (a) -- (b) ,
    (b)-- [scalar](c),
    (c)-- [] (d),
    (d) --[scalar] (o1)
    };
    \end{feynman}
  \end{tikzpicture}
 + ...\right\} \nonumber\\ & & \nonumber\\
  & = &  \lambda_d e^{r(t-t')} \int_{0}^{t-t'} e^{-(r + \lambda_d)\tau} I_0\left(2\sqrt{\beta\lambda_d \tau (t-t'-\tau)}\right) d\tau,
\end{eqnarray}
\end{widetext}
where $I_0$ and $I_1$ are the modified Bessel function of the first kind. These propagators are the building block of the theory and they must be taken into account for the calculation of observables. Imposing in the following the initial conditions $( N(0), M(0)) =(N_0, 0 )$, the mean number of neutrons and precursors can directly be written,
\begin{equation}
    \langle N(t) \rangle = N_0 \times \Sigma_{NN}(t,0)
\end{equation}
\begin{equation}
    \langle M(t) \rangle = N_0 \times \Sigma_{NM}(t,0)
\end{equation}

Imposing the initial condition $( N(0), M(0)) =(N_0, 0 )$, the variance of the neutron population may symbolically be written,
\begin{eqnarray}
    & & \langle N^2(t) \rangle_c   =  \nonumber\\ & & 2 \lambda_1 N_0 
    \begin{tikzpicture}[baseline=(a)]
    \begin{feynman}[inline=(a)]
      \vertex (a);
      \vertex [right= 0.5 cm of a,blob](b) {};
      \vertex [above left=0.5 cm of a,blob](f1) {};
      \vertex [below left=0.5cm of a,blob](f2) {};
      \vertex [above left=0.7 cm of f1](ff1);
      \vertex [below left=0.7 cm of f2](ff2);
      \vertex [right=0.7 cm of b](o1);
    \diagram* {
     (ff1) -- (f1)  -- (a) --  (f2) -- (ff2),
    (a) -- (b) --  (o1)
    };
    \end{feynman}
  \end{tikzpicture} + 2 \lambda_2 N_0
      \begin{tikzpicture}[baseline=(a)]
    \begin{feynman}[inline=(a)]
      \vertex (a);
      \vertex [right= 0.5 cm of a,blob](b) {};
      \vertex [above left=0.5 cm of a,blob](f1) {};
      \vertex [below left=0.5 cm of a,blob](f2) {};
      \vertex [above left=0.7 cm of f1](ff1);
      \vertex [below left=0.7 cm of f2](ff2);
      \vertex [right=0.7 cm of b](o1);
    \diagram* {
     (ff1) --  (f1)  -- [scalar] (a) -- [scalar] (f2) -- (ff2),
    (a) -- [scalar] (b) --  (o1)
    };
    \end{feynman}
  \end{tikzpicture}
\end{eqnarray}
whereas for the precursors, one has,
\begin{eqnarray}
    & & \langle N^2(t) \rangle_c   =  \nonumber\\ & & 2 \lambda_1 N_0 
    \begin{tikzpicture}[baseline=(a)]
    \begin{feynman}[inline=(a)]
      \vertex (a);
      \vertex [right= 0.5 cm of a,blob](b) {};
      \vertex [above left=0.5 cm of a,blob](f1) {};
      \vertex [below left=0.5cm of a,blob](f2) {};
      \vertex [above left=0.7 cm of f1](ff1);
      \vertex [below left=0.7 cm of f2](ff2);
      \vertex [right=0.7 cm of b](o1);
    \diagram* {
     (ff1) -- [scalar] (f1)  -- [] (a) -- []  (f2) -- [scalar] (ff2),
    (a) -- [] (b) --  (o1)
    };
    \end{feynman}
  \end{tikzpicture} + 2 \lambda_2 N_0
      \begin{tikzpicture}[baseline=(a)]
    \begin{feynman}[inline=(a)]
      \vertex (a);
      \vertex [right= 0.5 cm of a,blob](b) {};
      \vertex [above left=0.5 cm of a,blob](f1) {};
      \vertex [below left=0.5 cm of a,blob](f2) {};
      \vertex [above left=0.7 cm of f1](ff1);
      \vertex [below left=0.7 cm of f2](ff2);
      \vertex [right=0.7 cm of b](o1);
    \diagram* {
     (ff1) -- [scalar]  (f1)  -- [scalar] (a) -- [scalar] (f2) --[scalar]  (ff2),
    (a) -- [scalar] (b) --  (o1)
    };
    \end{feynman}
  \end{tikzpicture}
\end{eqnarray}

==> old/old_2_field_approach.tex <==
\section{ A Field theoretic formulation of neutron physics}
\label{sec:FieldFormulation}
{ \color{red}
Branching processes are among the simplest models capable of characterizing the complex phenomenology of the evolution of the neutron population in fissile materials (REFS). These processes are also known to display a second order phase transition between an active and an inactive state (REFS). This has a direct and practical transcription in the realm of neutron physics, for the phase transition translate into the formation of self-sustained fission chain reactions or  criticality, at the core root of nuclear reactors operations. The exponential increase or decrease of the neutron population corresponding to the conditions of the apparitions of self-sustained chains is controlled by a single parameter, the reactivity $\rho$ of the medium.   

Although branching processes are an invaluable tool to study the criticality of a nuclear reactor, this basic modelling is of course insufficient to properly encompass the complexity and variety of phenomena occurring in a nuclear reactor, especially when the latter is operating at a significant power level. A proficient tool for the analysis of nuclear reactor stability is to superimpose on the branching process a stochastic noise coming from the different noise sources that can alter the initial model. In other words, one suppose that the overall neutron population can be decoupled into
\begin{itemize}
    \item a smoothly varying neutron field $N(t)$. It correspond to the measured field observed in a reactor (through the operating power level for instance) and is only sensitive to the global reactivity $\rho$ of the reactor;
    
    \item a random source of noise $\eta(t)$, source of perturbations and driven by unknown or at least unspecified phenomena. 
\end{itemize}
}
The random noise source term can be added to the mean field equation derived from the branching process. The latter then is transformed into a Stochastic Differential Equation (SDE),
\begin{equation}
\label{LangevinEquation}
    \cfrac{d N(t)}{dt} = \rho N(t) + \eta(t).
\end{equation}

Any observable quantity $\mathcal{O}[N]$ must be averaged over all possibles configurations for the noise term. This is formally achieved by performing a functional integration over the noise probability functional $P[\eta]$: 
\begin{equation}
\label{observable}
    \langle \mathcal{O}[N] \rangle \, \propto \, \int \mathcal{D}\eta \, \mathcal{O}[N] \, P[\eta].
\end{equation}

Building on the seminal work of Janssen \cite{janssen1976} and De Dominicis \cite{dominicis1976}, one can take advantage of the structure of the problem to develop a field-theoretic formulation of the model, simplifying greatly the calculation of observables. 

\subsection{The response functional formalism}
\label{subsec:ResponseFunctional}

The development of the field-theoretic version of the present model starts by noting that the $N$ appearing in equation \ref{observable} is constrained to be a solution of equation \ref{LangevinEquation}. The constraint (valid for all $t$),
\begin{equation}
    \label{constraint_N}
    \mathcal{C}[N] \, = \, \left\{\frac{dN(t)}{dt} \, - \, \rho \, N(t) \,  -  \, n(t)\right\} = 0,
\end{equation}
can be enforced with the help of a functional version of the resolution of the identity \cite{cardy_tauber},
\begin{equation}
    1 = \int \mathcal{D}N \, \prod_t  \delta \left( \mathcal{C}[N] \right).
\end{equation}
Performing a (functional) Fourier transformation, one can write,
\begin{eqnarray}
\label{constrained_field}
    1 & = & \int \mathcal{D}[i\Nt] \int \mathcal{D}N \, e^{- \int dt \Nt(t) \, \mathcal{C}[N]} \nonumber\\
    & = & \int \mathcal{D}[i\Nt] \int \mathcal{D}N \, e^{- \int dt \Nt(t) \, \left( \frac{dN(t)}{dt} \, - \, \rho \, N(t) \,  -  \, \eta(t)\right)},
\end{eqnarray}
where the purely imaginary auxiliary field $\Nt(t)$, known as the Martin-Siggia-Rose response field \cite{martin_siggia_rose} has been introduced. Inserting this Fourier transformed identity back into equation \ref{observable}, one obtains,
\begin{eqnarray}
\label{observable2}
    \langle \mathcal{O}[N] \rangle & \propto & \int \mathcal{D}[i\Nt] \int \mathcal{D}N \left\{ e^{- \int \Nt(t)  \left( \frac{d}{dt}  -  \rho   \right)N(t) \, dt} \right. \nonumber \\ 
    & \times &\mathcal{O}[N] 
   \left.  \times  \int \mathcal{D}\eta \, e^{\int \Nt(t) \eta(t) dt} P[\eta] \right\}.
\end{eqnarray}
To go further, one needs to integrate over $\eta$ and thus specify the probability functional to which it is associated. In the following, it will be supposed that at any given moment in time, the noise possesses a Gaussian probability distribution 
\begin{equation}
\label{noise_proba}
    P[\eta] \propto e^{ -\frac{1}{4}\int \eta(t) \Gamma^{-1} \eta(t) \, dt }
\end{equation}
with zero mean $\langle \eta(t) \rangle = 0$ and a variance given by, 
\begin{equation}
    \langle n(t) n(t') \rangle = 2 \Gamma(N) \delta(t - t').
\end{equation} 
Note that an explicit dependence of the correlation function $\Gamma(N)$ to the global power level (i.e. $N(t)$) is to be expected on physical ground : the expected noise in a reactor indeed is dependent on the operating power level.

Imposing a Gaussian profile has the merit of making the integral over the noise in equation \ref{observable2} tractable. One has,
\begin{equation}
\int \mathcal{D}n \, e^{\int \Nt(t) n(t) dt} P[n] \propto e^{ \Gamma \Nt^2}.
\end{equation}
Inserting this results into equation \ref{observable2}, one finally arrives at an expression that solely depends on the variance of the noise probability distribution: 
\begin{equation}
\label{observable_final}
    \langle \mathcal{O}[N] \rangle \, = \mathcal{N}  \,  \int \mathcal{D}[i\Nt] \int \mathcal{D}N \, \mathcal{O}[N] \, 
    e^{- \mathcal{S}[N,\Nt]},
\end{equation}
where both a a normalisation factor $\mathcal{N}$ and the so-called \textit{response functional} have been introduced,
\begin{equation}
\label{response_functional}
     \mathcal{S}[N,\Nt] = \int \left\{\Nt(t)  \left( \frac{d}{dt} - \rho \right)N(t) - \Nt(t) \Gamma \Nt(t)\, \right\} dt.
\end{equation}
One could even go further and add another constraint on the model of equation \ref{constraint_N} to impose an initial condition for the field $N(t)$. Imposing that $N(t_0) = N_0$, one can show that the response functional becomes,
\begin{eqnarray}
\label{response_functional_initial_cond}
     \mathcal{S}[N,\Nt]  & \, & = \int \left\{  \Nt(t)  \left( \frac{d}{dt} - \rho \right)N(t)          \right.\nonumber\\
      && \left. -  \Nt(t) \, \delta(t-t_0) \, N_0   -   \Nt(t) \Gamma \Nt(t)\, \right\} dt.
\end{eqnarray}


==> old/old_6_feedback.tex <==
\section{Addition of counter-reactions - Directed percolation }
\label{sec:directed_percolation}

Up until now, the response functional formalism was used to retrieve most of the main results well known in nuclear reactor physics. Starting from the mean field equations derived from an underlying microscopic branching process, the proposed approach was capable of retrieving with relative ease the main results one would usually derive from solving the associated mean field equations.  

But because it is built on a macroscopic level of description, the principal advantage of the present field-theoretic approach has not been exploited yet: the formalism can easily incorporate effects for which a microscopic description is not available. In reactor physics, this is for instance the case of the feedback mechanisms applying on the neutron population in a reactor operating a high power (Doppler effect, Xenon poisoning, etc.). These phenomena are a central aspect of the stability of nuclear reactors but their detailed modelling is generally difficult to implement in a microscopic neutron balance.

Because the basic object of the field-theoretic approach proposed in this paper is already the coarse grain field $N(t)$, the introduction of, at least, a phenomenological model is much easier. Although now a direct link between the mean field equations and an underlying stochastic process is lost, one still is capable of extracting information about the moments associated to the neutron population distribution.  

One of the most paradigmatic feedback effect affecting the neutron population, and a key element in the study of reactors stability, is the Doppler broadening effect associated to the capture resonances of $^{238}$U. This effect originates from an increase in temperature observed in fissile materials when the neutron population increases. This induces a kinematic broadening of all of the resonant reactions in the medium, in particular the resonant capture of $^{238}$U (in low enriched reactors). As a consequence, when the temperature increases, more and more neutrons ends up being captured by the medium and the overall population is pulled back towards the reference operating power. The same mechanism applies in reverse when the temperature decreases.  

 This phenomenon is quite difficult to include in the microscopic branching process followed by the neutron population but can be quite straightforwardly implemented under the form of a restoring force of the type $\sigma N(N - N_{\text{ref.}})$ in the diffusion equation \footnote{under the assumption that the characteristic time associated to the Doppler broadening process is much faster than the mean generation time of the neutron population.} \cite{bell_glasstone}. The resulting equation can thus be written,  
\begin{equation}
    \label{stoch_diffusion_doppler}
    \frac{\partial }{ \partial t} N(\vec{x},t) - D ( \nabla^2 + r)  N(\vec{x},t)  +  \sigma N^2(\vec{x},t)  = 0,
\end{equation}
where the shifted parameter $ r = (\rho + \sigma N_{\text{ref.}})/D$ has been introduced, for convenience.

The response functional and the resulting theory to which this equation is associated has been extensively studied. It corresponds to the functional of the \textit{directed percolation} universality class \cite{janssen2004}, \cite{tauber_2005}:
\begin{equation}
    \mathcal{S} = \int d^d \vec{x} \int dt \Nt \left( \partial_t - D ( \vec{\nabla}^2 + r)  \right) N + \sigma \Nt N^2 - \lambda \Nt^2 N  .
\end{equation}

The inclusion of the term $\sigma N^2$ has a strong impact on the structure of the theory, for now the two following processes are allowed,
\begin{equation*}
    2 \lambda \begin{tikzpicture}[baseline=(a)]
    \begin{feynman}[inline=(a)]
      \vertex (a);
      \vertex [above left=of a](f1);
      \vertex [below left=of a](f2);
      \vertex [right=of a](o1);
    \diagram* {
    (f1) --[anti fermion] (a) --[fermion] (f2),
    (a) --[anti fermion] (o1)
    };
    \end{feynman}
  \end{tikzpicture} \hspace{2 cm} 2 \sigma
      \begin{tikzpicture}[baseline=(a)]
    \begin{feynman}[inline=(a)]
      \vertex (a);
      \vertex [above right=of a](f1);
      \vertex [below right=of a](f2);
      \vertex [left=of a](o1);
    \diagram* {
    (f1) --[fermion] (a) --[anti fermion] (f2),
    (a) --[fermion] (o1)
    };
    \end{feynman}
  \end{tikzpicture}
\end{equation*}
as well as their combination, i.e. the loop diagram, 
\begin{equation}
    4 \sigma \lambda \, 
    \begin{tikzpicture}[baseline=(a)]
    \begin{feynman}[inline=(a)]
      \vertex (z);
      \vertex [right=of z](a);
      \vertex [right=of a] (b);
      \vertex [above left=of a](f1);
      \vertex [below left=of a](f2);
      \vertex [right=of b](o1);
    \diagram* {
     (z) --[anti fermion] (a) 
     -- [fermion,half left] (b)
     -- [fermion,half left] (a),
    (b) --[anti fermion] (o1)
    };
    \end{feynman}
  \end{tikzpicture} \, ,
\end{equation}
whose contribution leads to badly divergent behaviours of two different types \cite{tauber_2005}:
\begin{itemize}
    \item a divergence is observed in dimension $d > 2$, because the momentum  associated to the loop is not constrained by any conservation rule. It's integration thus runs over theoretically infinite momenta and therefore include small distances, short time unbounded fluctuations of the neutron population. This is a paradigmatic example of an Ultra-Violet (UV) divergence.  
    
    \item another and more serious divergence occurs in dimension $d <4$. An Infrared (IR) divergence is observed in the long time, long distance limit. The highest dimension $d_c = 4$ for which the divergence is observed is called the \textit{critical dimension} of the problem.   
\end{itemize}

Both types of divergences can be eliminated through the well-known renormalization procedure \cite{Delamotte_2004}, which, in essence, consists in the application of successive spatio-temporal scaling transformation on the problem, so that the small distance and UV divergent fluctuations be truly integrated over. The true macro-scale description of the problem is obtained at a fixed point of the iterated scaling process which generally has the induced benefit of taming the residual IR divergence of the problem. The whole renormalization procedure leaves the system with two fundamental characteristics:
\begin{itemize}
    \item The asymptotic behaviour of the theory does not depend on the fine grain details and, in particular, on the precise origin of the phenomena at play. The resulting theory is \textit{universal}.
    
    \item Because the theory resulting from the renormalization procedure is derived at a fixed point of a spatio-temporal scaling transformation, the observables extracted from it will typically present power law behaviours. An imprint of the system's fluctuations will generally subsist, through characteristic \textit{critical exponents} whose values differ from the usual predictions of the mean field theories. In other words, mean field theory breaks down because of the collective phenomena observed at the critical point. Only the renormalized field theoretic description of the system can correctly describe the evolution of observables in the vicinity of the critical point. 
\end{itemize}


{\color{red} Some consequences are discussed below bla bla   }

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{ 0D model }

{\color{red}  
\begin{itemize}
    \item Mean number of neutrons : can we simply use the $\beta$ exponent ? $N \propto (-r)^\beta$ with 
       \begin{equation}
           \beta = 1 - \frac{\epsilon}{6} (\epsilon= d - d_c)
       \end{equation}
       No experimental consequence can be envisaged. Neither r nor sigma can be used to verify the proportinality between power and r/sigma. A calculation with an external source maybe ? Can the RG procedure be done with an external source ?  
       
     \item Variance : ?? 
     
     \item Comment eventually on percolation probability (= extinction probability) in the 0D model... 
     
     \item Any other observable ? Relaxation time might have something to do with the $\alpha$ exponent 
     
     \item  A model with precursors might be a nice refinement : might not be multi-species DP though because the precursors are not affected by the Doppler (?). 
\end{itemize} 
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{3D observables}

{\color{red} 

\begin{itemize}
    \item Mainly spatial correlations ? How to "use" the correlation length $\xi$ properly (what's the shape, $\exp( r/\xi)$ ?)? Can we conclude on neutron clustering ?
    
    \item Change in the typical cosine profile observed in reactors ? Is it possible to have an idea about that ?
    
    \item Boundary DP  ? \\
    Janssen H K, Schaub B, and Schmittmann B 1988 Z. Phys. B 72 111\\
    Howard M, Frojdh P, and Lauritsen K B 2000 Phys. Rev. E 61 167
\end{itemize}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{The DP conjecture}

{\color{red} 
The critical behaviour of the problem might be different with a more detailled modelling of the neutron population : energy, exponential jumps etc, finite size effect and quenched disorder...

The DP conjecture \cite{Hinrichsen2000} state that the DP transition quite generally reveals itself in every systems for which  
\begin{itemize}
    \item The model displays a continuous phase transition from a fluctuating active phase (neutrons alive) into a unique absorbing state (no neutrons).
    \item The transition is characterized by a positive one-component order parameter (survival probability).
    \item The dynamic rules involve only short-range processes.
    \item The system has no special attributes such as additional symmetries or quenched randomness
\end{itemize}

So that it might indeed shows up in neutronics ... 
}

